Exploring Covariate and Concept Shift for Detection and Calibration of Out-of-Distribution Data

Moving beyond testing on in-distribution data works on Out-of-Distribution (OOD) detection have recently increased in popularity. A recent attempt to categorize OOD data introduces the concept of near and far OOD detection. Specifically, prior works define characteristics of OOD data in terms of detection difficulty. We propose to characterize the spectrum of OOD data using two types of distribution shifts: covariate shift and concept shift, where covariate shift corresponds to change in style, e.g., noise, and concept shift indicates a change in semantics. This characterization reveals that sensitivity to each type of shift is important to the detection and confidence calibration of OOD data. Consequently, we investigate score functions that capture sensitivity to each type of dataset shift and methods that improve them. To this end, we theoretically derive two score functions for OOD detection, the covariate shift score and concept shift score, based on the decomposition of KL-divergence for both scores, and propose a geometrically-inspired method (Geometric ODIN) to improve OOD detection under both shifts with only in-distribution data. Additionally, the proposed method naturally leads to an expressive post-hoc calibration function which yields state-of-the-art calibration performance on both in-distribution and out-of-distribution data. We are the first to propose a method that works well across both OOD detection and calibration and under different types of shifts. View project page at https://sites.google.com/view/geometric-decomposition.

==> table/ood_results2.tex <==
\begin{table*}
\centering
\resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|c|c|ccc}  
        \toprule
        AUROC$\uparrow$&  Score Functions & ID:CIFAR100& \multicolumn{3}{c}{ID:CIFAR10}\\
        \midrule
        &  & Far  & Near & Near& Far\\
        
        &  & SVHN  & CIFAR100 & CIFAR10C & SVHN \\
        \midrule
        \multirow{3}{*}{Vanilla Wide-ResNet-28-10} 
        & MSP~\citep{hendrycks2016baseline}  & 77.37$\pm$2.25 &  88.93$\pm$0.37 & 70.58$\pm$0.59 & 93.66$\pm$1.79\\
        
        & Energy~\citep{liu2020energy} & 79.48$\pm$2.91 &  88.84$\pm$0.44 &70.60$\pm$0.52&94.39$\pm$2.30\\
        
        \citep{zagoruyko2016wide}& Mahanobis~\citep{lee2018simple} &84.37$\pm$4.56 &  87.63$\pm$1.19 & 68.38$\pm$0.50 & 93.08$\pm$6.02\\
        
        & GMM Density~\citep{mukhoti2021deterministic} & 85.67$\pm$2.02 &  90.98$\pm$0.24 &75.71$\pm$0.80 & 97.68$\pm$0.38\\
        
        \midrule
        DUQ~\citep{van2020uncertainty} & Kernel Distance & $-$&  85.92$\pm$0.35* & $-$ &93.71$\pm$0.61*\\
        
        SNGP~\citep{liu2020simple} & SoftMax Entropy & 85.71$\pm$0.81* &  91.13$\pm$0.15* & $-$&94.0$\pm$1.30*\\
        
        DDU~\citep{mukhoti2021deterministic} & GMM Density  & 87.32$\pm$0.77 & 90.69$\pm$0.42 &76.00$\pm$0.00 &97.12$\pm$1.21 \\
        
        5-Ensemble~\citep{lakshminarayanan2016simple} & SoftMax Entropy & 79.54$\pm$0.91* &  92.13$\pm$0.02*& $-$ &97.73$\pm$0.31*\\
        \midrule
        Ours: $\alpha(x)$-only & $h(y,x)$& 83.75$\pm$3.30$_h$ & 92.28$\pm$0.15$_h$ & 77.00$\pm$0.00$_h$ &97.56$\pm$0.90$_h$\\
        
        Ours: $\alpha$-$\beta$ & $\mathcal{U}$ &  \textbf{93.80$\pm$2.42}$_\mathcal{U}$ & \textbf{92.31$\pm$0.21}$_\mathcal{U}$ &\textbf{78.00$\pm$0.71}$_\mathcal{U}$&\textbf{99.54$\pm$0.08}$_\mathcal{U}$\\
        \bottomrule
    \end{tabular}
     }
    \caption{\textbf{AUROC $\uparrow$ for Near and Far OOD detection}. Results are averaged over 5 runs. Our $\alpha(x)$ only model is the same as Generalized ODIN~\citep{hsu2020generalized} without its input processing.* denotes results from~\cite{mukhoti2021deterministic}. }
    \label{tab:ood_results}
\end{table*}


